Predicting and Understanding Human Action Decisions during Skillful Joint-Action via Machine Learning and Explainable-AI

This study uses supervised machine learning (SML) and explainable artificial intelligence (AI) to model, predict and understand human decision-making during skillful joint-action. Long short-term memory networks were trained to predict the target selection decisions of expert and novice actors completing a dyadic herding task. Results revealed that the trained models were expertise specific and could not only accurately predict the target selection decisions of expert and novice herders but could do so at timescales that preceded an actor's conscious intent. To understand what differentiated the target selection decisions of expert and novice actors, we then employed the explainable-AI technique, SHapley Additive exPlanation, to identify the importance of informational features (variables) on model predictions. This analysis revealed that experts were more influenced by information about the state of their co-herders compared to novices. The utility of employing SML and explainable-AI techniques for investigating human decision-making is discussed.

==> Sections/acknowledgements.tex <==
\section*{Acknowledgments}
The authors thank Cassandra Crone for data coding, and Lilian Rigoli, Gaurav Patil, Patrick Nalepka, Elliot Saltzman, Mark Dras, Erik Reichle, Simon Hosking, Christopher Best, James Simpson and Roberto Pellungrini, for their collaborative support. Fabrizia Auletta's was supported by a Industrial and International Leverage Award from University of Bristol and an International Research Excellence Scholarship from Macquarie University. This research was also supported by an Australian Research Council Future Fellowshoip (FT180100447) awarded to Michael Richardson and Australian Department of Defence, Science and Technology group (MyIP8655 and HPRNet ID9024).

\section*{Author Contributions}
 FA, MB, RK and MR were all involved in conceptualization, formulation and assessment of study findings, as well as manuscript preparation. FA, MB and MR contributed to data modeling. KR and MR designed and developed the herding task employed and were lead investigators on the project that collected the original data. The authors have no competing interests related to the research presented here. Correspondence should be addressed to Michael J Richardson (michael.j.richardson@mq.edu.au) or Mario di Bernardo (mario.dibernardo@unina.it).
